Towards Optimizations of Quantum Circuit Simulation for Solving Max-Cut Problems with QAOA

Quantum approximate optimization algorithm (QAOA) is one of the popular quantum algorithms that are used to solve combinatorial optimization problems via approximations. QAOA is able to be evaluated on both physical and virtual quantum computers simulated by classical computers, with virtual ones being favored for their noise-free feature and availability. Nevertheless, performing QAOA on virtual quantum computers suffers from a slow simulation speed for solving combinatorial optimization problems which require large-scale quantum circuit simulation (QCS). In this paper, we propose techniques to accelerate QCS for QAOA using mathematical optimizations to compress quantum operations, incorporating efficient bitwise operations to further lower the computational complexity, and leveraging different levels of parallelisms from modern multi-core processors, with a study case to show the effectiveness on solving max-cut problems.

==> contents/chap2.tex <==
%\section{Preliminaries}
\section{Background and Related Work}
\label{chap:related_work}
This work is dedicated to accelerating the QAOA simulation speed for the max-cut problem. \sectionname~\ref{sec:math_maxcut} gives a theoretical background of the max-cut problem. \sectionname~\ref{sec:math_QAOA} further offers the theoretical and practical information of using the QAOA scheme for solving the max-cut problem. The related work of QAOA is given in Section~\ref{sec:related_work}, along with the discussion of the major difference between this work and the prior work. 
% This section provides a brief introduction to the Max-cut problem, including the objective function and approximation approaches, with corresponding mathematical representations in Section~\ref{sec:math_maxcut}. 
% The QAOA approach for optimizing the approximation ratio is then elaborated in Section~\ref{sec:math_QAOA}.


\subsection{The Max-Cut Problem}
\label{sec:math_maxcut}
% 話說我覺得 Max-Cut 比較適合放在 background 的部分 (好)
% A graph is composed of a set of points and edges. As shown in figure 3 (a), there are 7 vertices and 10 edges in the graph. It can be represented as $(V, E)$, where $V$ stands for the set of vertices and $E$ stands for the set of edges connecting two vertices. The goal of Max-Cut is to find a cut find the cut in a given graph such that the number of edges intersected by the cut is the maximum. For exmample, figure 3 (b) is the Max-Cut of figure 3 (a).

% C 老師的版本
%The Max-Cut problem is a NP-complete combinatorial optimization on graphs. A graph is composed of a set of vertices and edges. Each graphs can be represented as $(V, E)$, where $V$ represents the set of vertices and $E$ represents the set of edges connecting pairs of vertices. The goal of Max-Cut is to find a cut in a given graph such that the number of edges intersected by the cut is maximized. The objective function of Max-Cut can be formulated as below
% $$ C(x) = \sum_{(i,j) \in E} (1 - x_i * x_j) $$
% where x is N-bit string, each bit $x_i$ corresponds to a point on the graph. The cost function can be reduced to cost Hamiltonian by the relationship $x_i = Z_i $, where $Z_i$ is the pauli-Z gate.

The max-cut problem~\cite{maxcut1999} is regarded as an NP-hard combinatorial optimization problem that can be used in various application domains, such as network design, image segmentation, and statistical physics.
%\cmt{Please add the citation.}
Given an undirected graph $G = (V, E)$, where $V$ represents the vertices in $G$ and $E$ refers to the non-negative weighted edges, the goal of the max-cut problem is to find a cut in $G$ maximizes the number of edges between partitioned subsets of the vertices. To this end, a partition of the vertices into two sets $S$ and $\bar{S}$ ($V = S \cup \bar{S}$, $S \cap \bar{S} = \emptyset$), such that the cost function $C$ is maximized (i.e., the number of edges between $S$ and $\bar{S}$ is as large as possible). The cost function can be formulated as Equation~\ref{eq:cost_func}, where $w_{i,j} \in \mathbb{R}$ represents the weight of the edge $e_{i,j} \in E$ and $e_{i,j}$ is the edge between the vertices $v_i$ and $v_j$ ($v_i, v_j \in V$).

% The Max-Cut problem is a widely recognized NP-complete combinatorial optimization problem with various applications in fields such as network design, image segmentation, and statistical physics.
% Given an undirected graph $G = (V, E)$, where $V$ represents the set of vertices and $E$ represents the set of non-negative weighted edges, the objective is to find a cut in the graph that maximizes the number of edges crossing the partition.
% To achieve the goal, the problem involves determining a partition of the vertices $v \in V$ into two subsets, $S$ and $\bar{S} = V \setminus S$, such that the cost function $C$ is maximized. 
% The cost function $C$ can be formulated as Equation~\ref{eq:cost_func}, where $w_{i,j} \in \mathbb{R}$ represents the weight of the edge $e_{i,j} \in E$.

\begin{equation}
\begin{aligned}
\label{eq:cost_func}
%C(x) = \sum_{(i,j) \in E} (1 - x_i * x_j)
C(S, \bar{S}) = \sum_{i \in S, j \in \bar{S} } w_{i, j}
\end{aligned}
\end{equation}

An alternative way to evaluate the costs of different partitions is the introduction of a binarized vector, $\bm{z}$. The partition of the vertex $v_{i}$ into $S$ or the complement $\bar{S}$ can be represented by $\bm{z}_{i} \in \{{-1, 1\}}$. For example, considering a graph with six nodes on the left of \figurename~\ref{fig:example}, the $\bm{z}$ representation of the partition scheme on the right of the figure is $\bm{z} = (1, 1, -1, -1, -1, 1)$, where the nodes in the blue dashed circle are assigned to the set $S$ and the nodes in the green dashed circles belong to the set $\bar{S}$. The cost function can be then rewritten as Equation~\ref{eq:cost_func_sim}.

% As a result of the fundamental correlation between the set $S$ and its complement $\bar{S}$, the cost function $C$ can be significantly simplified.
% In the scenario of a graph $G$ with $|V|$ vertices, the partition of $V$ into $S$ or the complement $\bar{S}$ can be effectively represented by a binary string derived from a set $\bm{z} \in \{{-1, 1\}}^{|V|}$.
% For instance, consider a graph G comprising 6 nodes, as depicted in Figure~\ref{fig:example}.
% The corresponding binary string can be denoted as $\bm{z} = (1, 1, -1, -1, -1, 1)$, where the nodes in the blue block are assigned to set $S$ and the nodes in the green nodes belong to set $\bar{S}$.
% The cost function can be then characterized as Equation~\ref{eq:cost_func_sim}.

\begin{equation}
\begin{aligned}
\label{eq:cost_func_sim}
%C(x) = \sum_{(i,j) \in E} (1 - x_i * x_j)
C(\bm{z}) = \sum_{ \{i,j\} \in E} \frac{{w_{i,j}}}{2} {(1 - z_i z_j)}
\end{aligned}
\end{equation}



\begin{comment}
$$ H_c = \sum_{(i,j) \in E} Z_i Z_j $$
The cost Hamiltonian can be transformed to cost layer by the equation (X).
$$ U_c (\gamma) = \prod_{(i,j) \in E} e^{-i\gamma Z_i Z_j} $$
The Max-Cut problem is very common example when introducting QAOA because the problem is simple and each point and edge correspond to a unique qubit and a RZZ gate. For example, the figure X is the quantum circuit of graph in figure X.
\end{comment}

As the max-cut problem falls in the classification of NP-complete problems, approximation algorithms have been proposed to attain a good result for arbitrary graphs in a timely manner. The approximation ratio $r$ is used to 
quantify how \emph{good} the approximated result is\footnote{A noteworthy stochastic approximation algorithm was proposed in 1994~\cite{classic_r}, and it demonstrated an impressive approximation ratio of $r \approx 0.878$ in expectation. As of today, this method guarantees the best lower bound for classical algorithms without any additional constraints.}. 
The computation of $r$ is formulated as Equation~\ref{eq:approxi_val}, where the notation $max_{\bm{z}} C(\bm{z})$ is used to represent the optimal solution. Therefore, an approximation algorithm strives for finding the $r$ value approaching one. 


%As mentioned earlier, 
% Since the Max-Cut problem falls under the classification of NP-complete, indicating the absence of a polynomial-time algorithm to attain the optimal solution for arbitrary graphs.
% To overcome this limitation and achieve computational efficiency, approximation algorithms have been devised to identify reasonably good cuts, employing a parameter $r$ to denote the desired approximation ratio.
% As Equation~\ref{eq:approxi_val}, the notation $max_{\bm{z}} C(\bm{z})$ is used to represent the optimal solution.
% The evaluation of an approximation algorithm involves striving for $r$ to approach 1 as closely as possible, indicating a greater level of accuracy in the approximation.

\begin{equation}
\begin{aligned}
\label{eq:approxi_val}
\frac{C(\bm{z})} {max_{\bm{z}} C(\bm{z})} \geqslant r
\end{aligned}
\end{equation}

% In the past decades, several classical polynomial-time solutions have been explored for the Max-Cut problem, such as the greedy and random partition approaches.
% These intuitive algorithms can yield a lower bound of the approximation ratio $r$ that achieves an expectation value of 0.5.
% To exceed this expectation, a noteworthy stochastic approximation algorithm was proposed in 1994~\cite{classic_r}, demonstrating an impressive approximation ratio of $r \approx 0.878$ in expectation.
% It is accomplished by employing random rounding of the solution to a nonlinear programming relaxation and leveraging the properties of the symmetric positive semidefinite matrix, enabling the rational approximation to be found within polynomial time.
% As of today, this method still stands as the best approximation among classical algorithms without any additional constraints.
% Conversely, the field of quantum computing seeks to transcend and potentially surpass this significant milestone, with the QAOA emerging as one of the potential solutions.


\begin{figure}[htb!]
\centerline{\includegraphics[scale=0.27]{figures/example.pdf}}
\caption{An example of the max-cut problem on a six-vertex graph with weighted edges, where the maximum degree of any vertex is 3. (a) The three-regular graph. (b) The max-cut result of the corresponding example is equal to nine.}
\label{fig:example}
\end{figure}

%\subsection{Related Work of QAOA}
\subsection{Solving the Max-Cut Problem with QAOA}
\label{sec:math_QAOA}
% The quantum approximation optimization algorithm, abbreviated as QAOA, is a hybrid algorithm to solve combinatorial optimization problem. 

% The algorithm can map a problem in QUBO form to the quantum circuits that output a solution to the problem. The circuits is parameterized by the variables $(\beta, \gamma)$ and has a depth of p.

% The hybird algorithm can be regarded as the process to get better solution through updating the parameter $(\beta, \gamma)$. The process is composed of a series of rounds. In each round, the circuits paramterized by $(\beta, \gamma)$ is executed and output a solution. Then, the classical computer will update the parameter $(\beta, \gamma)$ according to the solution and the parameter is fed to the next round.

%The QAOA circuit is composed of two components: cost unitary and mixer unitary.
Quantum approximate optimization algorithm (QAOA) is considered to have a better approximation ratio than known polynomial classical algorithms for certain problems. QAOA adopts an iterative scheme to approximate solutions by updating the required parameters. The formal description and the modeling using the quantum gates for simulations are briefly introduced in the following subsections, in terms of solving the max-cut problem. 

% An iterative scheme is adopted by QAOA to approximate solutions via updating the required parameters for combinatorial optimization problems. The formal description and the modeling using the quantum gates for simulations are briefly introduced in the following subsections, in terms of solving the max-cut problem. 

\subsubsection{Formal Description} \label{sec:qaoacircuit} 
When applying QAOA for solving the max-cut problem, it is essential to obtain the two components, the \emph{cost unitary} $U(\hat{H}_{C}, \gamma)$ and the \emph{mixer unitary} $U(\hat{H}_{M}, \beta)$. 
The cost unitary is an operator directly associated with the problem to be solved. To obtain the cost unitary, the cost Hamiltonian $\hat{H}_{C} = C(x) \ket{x} \bra{x}$ should be determined first, where $C(x)$ is the cost function and $x$ is the bit string of the form ${\{0, 1\}}^N$, with $N$ representing the number of qubits and $N = |V|$. The cost Hamiltonian can be further simplified by removing unnecessary constant terms and negating the equation, which leads to Equation~\ref{eq:new_cost}, and the maximization problem is transformed into a minimization problem. 

% To apply the QAOA to solve the Max-Cut problem, the fundamentally primary components, it is essential to precisely define its fundamental components, namely the cost unitary $U(\hat{H}_{C}, \gamma)$ and the mixer unitary $U(\hat{H}_{M}, \beta)$.
% It is worth noting that the cost unitary is an operator directly associated with the problem solved.

% To obtain the cost unitary, we must pre-determine the cost Hamiltonian $\hat{H}_{C} = C(x) \ket{x} \bra{x}$, where $C(x)$ is the cost function and $x$ is the bit string of the form ${\{0, 1\}}^N$, with $N$ representing the number of qubits and $N = |V|$.
% Since QAOA involves updating the process to the cost function, the cost Hamiltonian can be further simplified by removing unnecessary constant terms and negating the equation.
% Consequently, the maximization problem is transformed into a minimization problem and the cost function can be rewritten as Equation~\ref{eq:new_cost}.

\begin{equation}
\begin{aligned}
\label{eq:new_cost}
C(z) = \sum_{\{i,j\} \in E} \frac{w_{i,j}}{2} z_i z_j
\end{aligned}
\end{equation}

% 該睡覺囉 
% 2.2 被註解掉了 是不要是濃縮
% 瞭
% 所以要變成 QAOA 介紹 再談 Max-Cut on QAOA 這樣？
% 逐步優化 應該是 調整 gamma 跟 beta? 那先這樣 晚安 保重

% 先說看著cost 調整杯，阿災
% 你再看看我這樣說有什麼不對

Given the cost function in Equation~\ref{eq:new_cost}, the cost Hamiltonian $\hat{H}_{C}$ and its cost unitary $U(\hat{H}_{C}, \gamma)$ can be expressed as Equation~\ref{eq:C}, where parameter $Z_i$ represents the unitary Pauli-Z operator acting on the $i$-th qubit, and it is achieved by the transformation $z_i \rightarrow Z_i$. The implementation of the cost unitary can be done by adopting a sequence of RZZ gates with parameters $w_{i,j}$ and $\gamma$.

% Through the reformulation of the cost function, the cost Hamiltonian $\hat{H}_{C}$ and its cost unitary $U(\hat{H}_{C}, \gamma)$ can be readily expressed as shown in Equation~\ref{eq:C}, where parameter $Z_i$ represents the unitary Pauli-Z operator acting on the $i$-th qubit, and it is achieved by the transformation $z_i \rightarrow Z_i$.
% %$z_i\rightarrow\frac{1}{2}(1-Z_i)$.
% To implement the cost unitary using quantum computing, it can be accomplished effortlessly by adopting a series of RZZ gates with parameters $w_{i,j}$ and $\gamma$.

\begin{equation}
\label{eq:C}
\begin{aligned}
\hat{H}_{C} = & \sum_{\{i,j\} \in E} \frac{w_{i,j}}{2} Z_i Z_j \\
U(\hat{H}_{C}, \gamma) = & \ e^{-i\gamma \hat{H}_{C}} = \prod_{\{i,j\} \in E}  e^{-i\gamma \frac{w_{i,j}}{2} Z_{i} Z_{j} }
\end{aligned}
\end{equation}

The mixer Hamiltonian $\hat{H}_{M}$ and its unitary operator $U(\hat{H}_{M}, \beta)$ are defined as Equation~\ref{eq:B}. The mixer Hamiltonian can be expressed by the Pauli-X operator and is independent of the cost functions.
The mixer unitary with parameters $\beta$ can be implemented by RX gates. 

% On the other hand, the mixer Hamiltonian $\hat{H}_{M}$ and its 
% corresponding unitary operator $U(\hat{H}_{M}, \beta)$ can be defined as Equation~\ref{eq:B}. 
% The mixer Hamiltonian can be expressed by Pauli-X operator and is fully independent of the cost functions.
% %utilized to maintain a specified subspace 
% In addition, the mixer unitary with parameters $\beta$ can often be represented using RX gates.

\begin{equation}
\begin{aligned}
\label{eq:B}
\hat{H}_{M} = & \sum_{i=0}^{n-1} X_i \\
U(\hat{H}_{M}, \beta) = & \  e^{-i\beta \hat{H}_{M}} = \prod_{j=1}^{n} e^{-i\beta X_{j}}
\end{aligned}
\end{equation}

The $p$-level QAOA circuit can be formulated as Equation~\ref{eq:QAOA} based on the developed cost and mixer unitary, where $\bm{\gamma} = (\gamma_1, \gamma_2, ..., \gamma_p)$ and $\bm{\beta} = (\beta_1, \beta_2, ..., \beta_p)$. For $i = 1, ..., p$, each $\gamma_i$ and $\beta_i$ takes a value in the interval $[0, 2\pi)$ and $[0, \pi)$, respectively. The symmetric superposition of quantum state $\ket{+}^{\otimes N}$ is initialized by applying Hadamard gates to $N$ qubits.


% With the cost and mixer unitary in place, the final state output by the $p$-level QAOA circuit can be formulated as shown in Equation~\ref{eq:QAOA}, where $\bm{\gamma} = (\gamma_1, \gamma_2, ..., \gamma_p)$ and $\bm{\beta} = (\beta_1, \beta_2, ..., \beta_p)$. 
% For $i = 1, ..., p$, each $\gamma_i$ and $\beta_i$ takes values in the interval $[0, 2\pi)$ and $[0, \pi)$, respectively. 
% The symmetric superposition of quantum state $\ket{+}^{\oplus N}$ is initialized by applying Hadamard gates to $N$ qubits.

\begin{equation}
\begin{aligned}
\label{eq:QAOA}
\ket{\bm{\gamma}, \bm{\beta}} = U(\hat{H}_{M}, \beta_p) U(\hat{H}_{C}, \gamma_p) \cdots 
 U(\hat{H}_{M}, \beta_1) U(\hat{H}_{C}, \gamma_1) \ket{+}^{\otimes N}
\end{aligned}
\end{equation}

The expectation value of the Hamiltonian $H_{C}$ in this quantum state can be determined by repeatedly measuring the final state in the computational basis, as shown in Equation~\ref{eq:Fp}.

\begin{equation}
\begin{aligned}
\label{eq:Fp}
Fp (\bm{\gamma}, \bm{\beta}) = \langle \bm{\gamma}, \bm{\beta} \mid C \mid \bm{\gamma}, \bm{\beta} \rangle
\end{aligned}
\end{equation}

An iterative optimization algorithm for updating the parameters, $\gamma$ and $\beta$ ($\gamma, \beta \in \mathbb{R}^p$), is adopted to determine the parameters on classical computers, such that the expectation value $Fp (\bm{\gamma}, \bm{\beta})$ can be converged, as shown in Equation~\ref{eq:Mp}. 

% To determine the optimal parameters $\gamma$ and $\beta$, where $\gamma, \beta \in \mathbb{R}^p$ such that the expectation value $Fp (\bm{\gamma}, \bm{\beta})$ can be converged, as indicated in Equation~\ref{eq:Mp}, an iterative optimization algorithm for updating these parameters is employed on the classical computer.

\begin{equation}
\begin{aligned}
\label{eq:Mp}
M_p = \min_{\bm{\gamma}, \bm{\beta}} F_p (\bm{\gamma}, \bm{\beta})
\end{aligned}
\end{equation}

% Finally, the approximation ratio is represented as Eqaution~\ref{eq:QAOA_ratio}.
\begin{equation}
\begin{aligned}
\label{eq:QAOA_ratio}
r = \frac{\min_{z} C(z)}{M_p}
\end{aligned}
\end{equation}

The corresponding approximation ratio is defined in Equation~\ref{eq:QAOA_ratio}. The approximation ratio of QAOA is correlated with the number of the QAOA circuit levels $p$. According to the Adiabatic Theorem~\cite{ori_qaoa}, the approximated result is proven to converge to the optimal solution when the $p$ value approaches infinity. Nonetheless, an increasing $p$ value will lead to the growth of the number of parameters $\bm{\gamma}$ and $\bm{\beta}$, incurring the overhead for searching the solution.
Several studies~\cite{crooks2018performance, level_numbers}, reporting a monotonically increasing and decreasing pattern for $\bm{\gamma}$ and $\bm{\beta}$ respectively, can be leveraged to develop strategies for searching the optimal set of the parameters.

% $\bm{\gamma}$ and $\bm{\beta}$ exhibit a monotonically increasing and decreasing pattern, respectively.
% That is, with a well-designed strategy, finding the optimal set of these parameters can be easily achieved.

% The approximation ratio of QAOA is positively correlated with the number of levels $p$.
% As $p$ approaches infinity, the result is proven to converge to the optimal solution according to the Adiabatic Theorem~\cite{ori_qaoa}.
% However, with increasing $p$, the number of parameters $\bm{\gamma}$ and $\bm{\beta}$ would also grow, potentially leading to an overhead in searching for the solution.
% Delightfully, several studies~\cite{crooks2018performance, level_numbers} have observed that $\bm{\gamma}$ and $\bm{\beta}$ exhibit a monotonically increasing and decreasing pattern, respectively.
% That is, with a well-designed strategy, finding the optimal set of these parameters can be easily achieved.

%In brief, QAOA can be referred to as simply Quantum Annealing QAA, which is an evolution of the quantum state.
%By applying the Suzuki-Trotter decomposition and properly adjusting the parameters for the evolution, the approximation formula is almost identical to Eqaution~\ref{eq:QAOA} with monotonically fine-tuned parameters $\bm{\gamma}$ and $\bm{\beta}$.

\begin{comment}
The QAOA is fundamentally composed of two primary components, including cost and mixer unitary. 
The cost Unitary, denoted as $U(\hat{H}_{C}, \gamma)$, is the unitary operator associated with the problem solved. 
To obtain the cost unitary, we must pre-determine the cost Hamiltonian $\hat{H}_{C}$ as Equation~\ref{eq:HC}, where $z$ is the bit string of the form ${\{-1, 1\}}^N$ and N XXX .

\begin{equation}
\begin{aligned}
\label{eq:HC}
\hat{H}_{C} = C(z) \ket{z} \bra{z}
\end{aligned}
\end{equation}

 The cost Hamiltonian is derived from the cost function like ~\ref{eq:cost_func_sim}. However, before transforming the cost function, we reduce some constant terms and negate the equation ~\ref{eq:cost_func_sim}, to turn the equation from maximization into minimization.

\begin{equation}
\begin{aligned}
\label{eq:cost_func_min}
C'(z) = \sum_{\{i,j\} \in E} \frac{w_{i,j}}{2} z_i z_j
\end{aligned}
\end{equation}

To transform the simplified cost function to the cost Hamiltonian, we can apply the transformation $ z_i \rightarrow Z_i $, where $Z_i$ is the unitary of Pauli-Z gate on i-th qubit and can be written as Equation~\ref{eq:Z}.

\begin{equation}
\begin{aligned}
\label{eq:Z}
Z_i = (-1) ^ {z_i+1} \ket{z} \bra{z}
\end{aligned}
\end{equation}

So cost Hamiltonian of Max-Cut problem becomes

\begin{equation}
\begin{aligned}
\label{eq:C}
\hat{H}_{C} = \sum_{\{i,j\} \in E} \frac{w_{i,j}}{2} Z_i Z_j
\end{aligned}
\end{equation}

The cost unitary for Max-Cut problem becomes

\begin{equation}
\begin{aligned}
\label{eq:UC}
U(\hat{H}_{C}, \gamma) = e^{-i\gamma \hat{H}_{C}} = \prod_{\{i,j\} \in E}  e^{-i\gamma \frac{w_{i,j}}{2} Z_{i} Z_{j} }
\end{aligned}
\end{equation}

We can implement the cost unitary by applying many RZZ gates of $\theta=w_{i,j} \gamma$. 
% The unitary of RZZ gate is $ R_{Z_iZ_j}(\gamma w_{i,j}) = e^{-i\gamma \frac{w_{i,j}}{2} Z_{i} Z_{j} }$

% check this to write the minimize formulation:
% ref: https://arxiv.org/pdf/1811.08419.pdf
% ref : https://arxiv.org/pdf/2009.01760.pdf

% [Chuan Chi Wang] Why p is larger get better results: https://quantumcomputing.stackexchange.com/questions/15391/why-qaoa-with-p-rightarrow-infty-gives-the-optimal-solution

% we may just write that `by applying QAA~\cite{} and the and Trotterization~\cite{}, the ratio → 1 when p → ∞`; 或者在這邊只提到 p 越大 r 越好, 會在下一小節交代細節
% In the ref, the gamma and beta in the Max-Cut problem, would monotonically increase and decrease, respectively.

%review: https://arxiv.org/pdf/2306.09198.pdf

The mixer Hamiltonian, $\hat{H}_{M}$ is independent of the cost function and is defined as 

\begin{equation}
\begin{aligned}
\label{eq:B}
\hat{H}_{M} = \sum_{i=0}^{n-1} X_i
\end{aligned}
\end{equation}

where the $X_i$ is the Pauli-X gate on the i-th bit. The mixer unitary is

\begin{equation}
\begin{aligned}
\label{eq:UB}
U(\hat{H}_{M}, \beta) = e^{-i\beta \hat{H}_{M}} = \prod_{j=1}^{n} e^{-i\beta X_{j}}
\end{aligned}
\end{equation}

The mixer unitary can be implemented by applying many RX gates of $\theta=\beta$.


Since the cost unitary and mixer unitary is known, the QAOA circuit is known. The definition of QAOA circuit is 

\begin{equation}
\begin{aligned}
\label{eq:QAOA}
\ket{\bm{\gamma}, \bm{\beta}} = U(\hat{H}_{C}, \gamma_p) U(\hat{H}_{M}, \beta_p) \cdots U(\hat{H}_{C}, \gamma_1) U(\hat{H}_{M}, \beta_1) \ket{+}^{\oplus N}
\end{aligned}
\end{equation}

The QAOA circuit is composed of p replica of cost unitary and mixer unitary. The number of p will affect the approximation ratio of the QAOA circuit. To understand the relationship between p and approximation ratio, let's pretend p is fixed and define the expectation of the p-level QAOA circuit as
% To understand the approximation ratio of QAOA algorithm, the expectation of p-level QAOA circuit $F_p$ is defined as

\begin{equation}
\begin{aligned}
\label{eq:Fp}
Fp (\bm{\gamma}, \bm{\beta}) = \langle \bm{\gamma}, \bm{\beta} \mid C \mid \bm{\gamma}, \bm{\beta} \rangle
\end{aligned}
\end{equation}

Since the expectation of a QAOA circuit is defined, the minimal expectation within a p-level circuit, $M_p$, is the minimum of the expectation of all possible p-level circuits

$$ M_p = \min_{\bm{\gamma}, \bm{\beta}} F_p (\bm{\gamma}, \bm{\beta}) $$

So the approximation ratio of when the number of level is p is

\begin{equation}
\begin{aligned}
\label{eq:ratio}
r = \frac{\min_{z} C'(z)}{M_p}
\end{aligned}
\end{equation}

It's crucial that the increase of p will improve the approximation ratio. There are two reasons. First, notice that the relationship $M_{p+1} \leq M_p$ is always hold since any p-level circuit can be transformed to the (p+1)-level circuit by appending a set of cost unitary with $\gamma=0$  and mixer unitary with $\gamma=0$ to the p-level circuit. Second, by Trotterization, which will be explained later, the following equation holds

\begin{equation}
\begin{aligned}
\label{eq:lim}
\lim_{p \rightarrow \infty} = \min_{z} C'(z)
\end{aligned}
\end{equation}

% 這裡
% The hybrid algorithm can be seen as a process of multiple iterations to improve the solution (i.e. find the lower energy state) by updating the parameters $(\beta, \gamma)$. In each iteration, the quantum circuits, with their parameters denoted as "$( \beta, \gamma)$," are run on either a quantum computer or a quantum simulator. Through this process, a solution is generated. The classical computer then updates the parameters $(\beta, \gamma)$ based on the obtained solution, which are subsequently used in the next iteration.

% The circuit is composed of a series of H gates on each qubits as a initialization. Each round is composed of two layers, cost layer and mixer layer. The definition of two layers are shown below.

% $$U_c (\gamma) = \prod e^{-i \gamma H_c}$$
% $$U_m (\beta) = \prod e^{-i \beta H_m}$$

% The $H_c$, cost Hamiltonian, is related to the problem solved. While the $H_m$, mixer Hamiltonian, is fixed to the following equation.

% $$H_m = \sum_{i \in [0,N)} X_i$$
\end{comment}

\begin{figure}[tb!]
    \centerline{\includegraphics[scale=0.36]{figures/circuit.pdf}}
    \caption{The quantum gates used in a single-level of QAOA.}
    \label{fig:circuit}
\end{figure}

    \subsubsection{Modeling for the QAOA Simulation} \label{sec:qaoacircuit} 
    A single-level QAOA circuit is a basic infrastructure for the iterative procedure of a multi-level QAOA circuit. The quantum gates of a single-level QAOA, which are used to solve the max-cut problem, are illustrated in \figurename~\ref{fig:circuit}. A three-layer structure is presented based on the formal description of the $p$-level QAOA circuit in \sectionname~\ref{sec:qaoacircuit}. The first layer is used to do the quantum state initialization, whereas the following two layers are applied iteratively to improve the quantum state and to approximate the optimal solution. An increasing $p$ value provides a better-approximated result. The solution searching process can be improved by adjusting the parameters $(\bm{\gamma}, \bm{\beta})$ of the cost and mixer layers at each level. The functionality of each layer is described as follows.

    % The quantum gates of a single-level of QAOA solving the max-cut problem is illustrated in \figurename~\ref{fig:circuit}. The first layer is for state initialization, and two additional layers are applied to iteratively improve the quantum state and approximate the optimal solution.
    % To achieve a better approximation, the level (or depth) of the cost and mixer layers is continuously increased.
    % By successfully adjusting the parameters $(\bm{\gamma}, \bm{\beta})$ of these layers at each level, the algorithm is able to refine its search, making QAOA a approach for various tasks.
    % The function of each layer is described as follows.

    \paragraph{\textbf{Initial layer}} This first layer initializes the quantum state, and one common implementation is to place Hadamard gates to the $N$-qubit system in $|0...0\rangle$ state. This superposition operation creates a quantum state where all possible combinations of 0 and 1 have equal probability amplitudes, leading to uniform superposition. The use of Hadamard gates for the initialization of quantum systems has been seen in several famous algorithms~\cite{grover, Bernstein, Simon}.
    
    % The initial layer constitutes the first step of QAOA and plays a crucial role in preparing a specific initial state to set the quantum state to efficiently explore the solution space.
    % One common approach to implement this layer is by applying a series of fundamental Hadamard gates to each $N$-qubit in $|0...0\rangle$ state.
    % This superposition operation creates a quantum state in which all possible combinations of 0 and 1 have equal probability amplitudes.
    % The resulting state, with its uniform superposition, serves as a solid starting point for QAOA.
    % The application of Hadamard gates for initialization has been well-established and applied in several famous algorithms~\cite{grover, Bernstein, Simon}.
    
    \paragraph{\textbf{Cost layer}} This layer is designed to implement the Hamiltonian of the cost function $\hat{H}_{c}$ with the quantum gates. The design should be done carefully for targeting different problems. For the max-cut problem, this layer encodes the connectivity and weights of a given graph into the quantum circuit. It is done by mapping each graph node to a qubit in the circuit, and the qubit size scales with the growth of the problem size. 
    Specifically, in this work, each graph edge is represented as a RZZ gate, where the target qubits correspond to the connected nodes and the weights influence the rotation angle of the RZZ gate. In other words, the RZZ gates represent whether the two qubits (graph nodes), $i$ and $j$, are in different subsets, and hence, this representation method can reflect the status of whether the corresponding edges are being cut or not.

    % By manipulating the $\gamma$ properly, the cost layer assigns different cost values to different quantum states, effectively capturing the objective solution of the Max-Cut problem.
    
    \paragraph{\textbf{Mixer layer}} This layer provides feasible states that correspond to those of the preceding gates. Mathematically, the mixer $\hat{H}_M$ is irrelevant to the cost function $\hat{H}_C$, resulting in a non-constant expectation of the objective function. This property offers an advantage in minimizing or maximizing the cost function using classical optimizers. As for the max-cut problem, the RX gates are frequently applied for each qubit within the mixer layer.
    
    % As the final step of a level of QAOA, the mixer layer is used to provide feasible states that correspond to the preceding gates.
    % Mathematically, the mixer $\hat{H}_M$ and the cost function $\hat{H}_C$ do not commute, resulting in a non-constant expectation of the objective function. 
    % This property offers an advantage in efficiently minimizing or maximizing the cost function using classical optimizers.
    % In the Max-Cut problem,  the RX gates are frequently applied for each qubit within the mixer layer.


\subsection{Related Work}
\label{sec:related_work}
% 引言：QAOA 是師承 QAA 的改版，透過將將ＱＡＡ的參數 改寫成 gamma 跟 beta，有著更好的 彈性適應性，解空間探索 (adaptability, flexibility, and versatility) ...
% 具備著這樣的良好特性，使得 QAOA 在 ＣＯＰ中被更深入地探討，並可以簡單區分成以下三個主軸
QAOA is one of the quantum optimization algorithms specifically for the combinational optimization problem. The following paragraphs introduce the studies of QAOA from different aspects: 1) algorithm improvement, 2) approximation result quality analysis, 3) noise and error analysis, and 4) quantum circuit simulators. The last paragraph discusses the major difference between this work and the existing works. 

% The QAOA can be comprehended as a discretized version of quantum annealing, featuring substantial parallels with the Quantum Adiabatic Algorithm (QAA).
% By extending the parameter requisites of QAA to include the $\gamma$ and $\beta$  parameters inherent in QAOA, it can alleviate the concern of entrapment within the false minimum, consequently elevating the exploration of solution spaces.
%The enhancement in adaptability, flexibility, and versatility endows QAOA with a distinctive advantage in dealing with the domain of combinatorial optimization problems.
% These advantages endow QAOA with a distinctive advantage in dealing with the domain of combinatorial optimization problems.
% To surmount potential challenges within this field, the research subjects can be methodically structured in the forthcoming paragraphs.

%1. Initial parameter and optimizer (sec 3.1, sec 3.2, sec 3.3.32)
\paragraph{\textbf{Algorithm improvement}} A number of algorithms have been proposed to expedite the convergence rate of the approximation ratio. For example, QAOA+~\cite{QAOAplus} and ma-QAOA~\cite{multiangle} added extra parameters for the cost and mixer layers to improve the approximation ratio. CD-QAOA~\cite{CD_QAOA} and DC-QAOA~\cite{DC_QAOA} employed the counter-diabatic operator to minimize circuit depth while maintaining high solution quality. QAOA frameworks~\cite{zhu2022adaptive, a12020034, a15060202} have been presented to consider both hardware capabilities and problem-specific constraints. Regarding parameter optimization, efforts have been made to explore proper initial parameterizations~\cite{level_numbers, init_QAOA1, init_QAOA2}. The selection of QAOA optimizers is also studied in \cite{gradient_optimizer, QAOA_minimizers, QAOA_opts}.

% In the endeavor to elevate performance metrics and expedite the rate of convergence regarding the approximation ratio, a range of variations of QAOA is put forward.
% Intuitively, QAOA+~\cite{QAOAplus} and ma-QAOA~\cite{multiangle} proposed to increase the number of parameters for the cost and mixer layer to increase the approximation ratio.
% CD-QAOA~\cite{CD_QAOA} and DC-QAOA~\cite{DC_QAOA} employ the counter-diabatic operator to effectively minimize circuit depth while maintaining high solution quality.
% As hardware capabilities and problem-specific constraints are increasingly integrated, they give rise to a multitude of distinct QAOA frameworks~\cite{zhu2022adaptive, a12020034, a15060202}. 
% In the domain of parameter optimization, several investigations are dedicated to the quest for well-suited initial parameterizations~\cite{level_numbers, init_QAOA1, init_QAOA2}.
% Concurrently, the selection of QAOA optimizers garners attention within certain research teams~\cite{gradient_optimizer, QAOA_minimizers, QAOA_opts}.


%2. The approximate ratio for different constraints (sec 3.4, 提到經驗法則)
\paragraph{\textbf{Approximation quality analysis}}
% \textbf{Solution Quality.}
Mathematical frameworks play a vital role in QAOA-based approximations, and it is important to analyze theoretical boundaries associated with various QAOA designs, as well as inherited capabilities and constraints. 
Studies have been done to estimate the lower bound for the approximation ratio of the max-cut problem on 2-regular and 3-regular graphs~\cite{ori_qaoa, maxcut_ratio1, maxcut_ratio2} when fixed-depth QAOA designs. Besides, the one-level optimized QAOA can provide an approximation~\cite{maxcut_ratio_with_d} that outperforms the lower bound of the best-known classical algorithm on different degrees of regular graphs~\cite{classical_ratio}. 
% As an aspect of research and scientific exploration, the establishment of mathematical frameworks plays a pivotal role in approximation algorithms.
% Consequently, delving into the analysis of the theoretical boundaries associated with QAOA facilitates a comprehensive understanding of its inherent capabilities and constraints. 
% This understanding further enables a comparative assessment with classical algorithms.
% By applying QAOA of a fixed depth, several studies~\cite{ori_qaoa, maxcut_ratio1, maxcut_ratio2} derived the lower bound for the approximation ratio in the Max-Cut problem on 2-regular and 3-regular graphs.
% For another aspect, the 1-level of optimized QAOA can provide an approximation~\cite{maxcut_ratio_with_d}, outperforming the lower bound of the best-known classical algorithm across varying degrees of regular graphs~\cite{classical_ratio}.
% 雖然這樣的研究成果，使得更多數值分析不同應用問題上被加以延續, 但更多的研究是伴隨著更多的限制
% 故此，Empirical evidence被視為有淺力的解決方案
% 其中, 經典的 Max-cut 問題被在不同條件下被數個research 全面地探討
% 這些真實運行的求解在 p足夠深度下，可以比ＧＷ算法有更好的近似值
% 不僅如此，近似值確實會隨著p值得提高單調地遞增
% While such research findings have propelled the continued application of mathematical analysis to various practical problems, they have been concurrently complemented by supplementary constraints. 
% Hence, empirical evidence is recognized as a pragmatic viable avenue for resolution. 
%\cmt{I removed some citations below. Please check the tex source see if they are so important that we need to cite them.}
Furthermore, the typical max-cut problem has been scrutinized under assorted conditions~\cite{ori_qaoa, Empirical}, with outcomes that can effortlessly outperform the performance of the GW algorithm~\cite{classic_r} even at shallow depths.
% Among these investigations, the typical Max-Cut problem has been scrutinized under assorted conditions~\cite{ori_qaoa, Empirical}, with outcomes that can effortlessly outperform the performance of the GW algorithm~\cite{classic_r} even at shallow depths.
% Furthermore, it is evident that the solution quality improves monotonically as the value of $p$ increases.

%3. Noise overhead (sec 3.5, 用傳統電腦模擬可以克服)
\paragraph{\textbf{Noise and error analysis}}
% {\textbf{Noise and Error Analysis.}
The QAOA approximation ratio has a positive correlation with the QAOA circuit levels when the QAOA computations are performed in an ideal environment. Unfortunately, as in the noisy intermediate-scale quantum (NISQ) era, quantum processors are not capable of fault tolerance and computational noise exists for a moderate number of qubits in the systems. This noise further causes the generation of erratic results. 
Compilation techniques are developed to minimize the noise and streamline gate utilization by translating the set of native gates used by the targeting quantum hardware~\cite{compile1, compile2, compile3, compile4, compile5}.
In addition, studies have shown that the fidelity and approximation ratio of the QAOA circuit tends to deteriorate with the increasing of the number of qubits and the circuit depth~\cite{compile5, increase_hazard2, increase_hazard3, increase_hazard4}.

% In an ideal scenario, the approximation ratio of QAOA exhibits a positive correlation with the circuit depth.
% However, during the Noisy Intermediate-Scale Quantum (NISQ) era, quantum computers have a moderate number of qubits but suffer from diverse sources of computational noise.
% This noise gives rise to discrepancies between anticipated computational outcomes and the actual results produced by quantum computers, ultimately diminishing their inherent advantages.
% In an effort to minimize the effect of noise and streamline gate utilization, compilation techniques have been proposed to translate the set of native gates used by the targeting quantum hardware~\cite{compile1, compile2, compile3, compile4, compile5}.
% % However, numerous studies have shown that the fidelity and approximation ratio of the QAOA circuit tends to deteriorate as the number of qubits and the depth increase~\cite{increase_hazard1, increase_hazard2, increase_hazard3, increase_hazard4}.
% Considering the substantial cost associated with accessing actual quantum hardware, this imposes constraints on the feasibility of implementing large-scale QAOA circuits, thereby impeding the progress within this research domain.

% In summary, 在不同實務的限制下，使用量子電腦來找到一組穩定的近似解 其實 不是一件容易的事, 尤其在large scale 的 量子計算更是如此
% 這樣的缺點反而使得 被視為潛力的 經驗法則 混亂不堪
% 相比而言，傳統電腦的模擬 卻能 避開 量子電腦的這個尚待技術優化的問題。
% 配合上使用 薛丁格 style 的 simulation, researchers 更能清楚地觀測病檢驗整個 QAOA 的過程
% 因此，本論文強調去更快的模擬出穩定的 QAOA 實驗，並讓 QAOA 在 組合優化問題的道路上 走更遠

\paragraph{\textbf{Quantum circuit simulators}}
General-purpose quantum circuit simulators are useful to evaluate the QAOA algorithms when physical quantum computers are absent or the noise brought by the physical quantum computers cannot provide reliable results. To accelerate the simulators running on classical computers, the multi-threaded approach is adopted by the prior work to utilize multicore processors (e.g., QuEST~\cite{QuEST} and Quantum++~\cite{quantum_plus2}). The single-instruction-multiple-data engines are used to accelerate the simulation speeds~\cite{qHiPSTER, projectQ, Cirq}. There are some works have been developed to unlock the computational power of the massive parallelism on GPUs~\cite{QuEST, cuQuantum}. 

% In the domain of quantum circuit simulation, significant research endeavors have been dedicated to enhancing efficiency and extending applicability with noise-free impact.
% Some studies have adopted a multi-threaded approach to optimize CPU utilization~\cite{QuEST, quantum_plus2}, while others have proposed additional vectorized operations, such as AVX, in various simulators~\cite{qHiPSTER, H_ner_2017, projectQ, Cirq}. 
% To leverage massive parallelism on GPUs, certain approaches~\cite{QuEST, cuQuantum} have been introduced to utilize the computational power of the thousands of available cores.
% Furthermore, in pursuit of cost-efficiently extending applicability, SSD-based and RDMA-based simulator leverages secondary storage devices and unused remote memory resources to enlarge the number of qubits.

\paragraph{\textbf{Discussion}}
This work focuses on the optimizations of the standard QAOA algorithm (in Algorithm~\ref{algo:standard_QAOA} that is adopted by the state-of-the-art simulator QuEST) to expedite the QAOA simulation speed for solving the max-cut problem. The optimizations are done in different perspectives: mathematical forms (\sectionname~\ref{sec:general_opt}), bitwise implementation scheme (\sectionname~\ref{sec:uGraph_opt}), and parallelization techniques (\sectionname~\ref{sec:avx_opt}). To the best of our knowledge, we are unaware of any other work that adopts such a comprehensive methodology (from theoretical algorithms to parallel processing) to accelerate the QAOA simulation speed for solving the max-cut problem. This work paves the way for solving the QAOA-based max-cut problem. 

% In summary, the practical constraints of quantum computers have led to confusion surrounding the once-promising empirical methodologies.
% Conversely, quantum circuit simulations on classical computers can sidestep these technological optimization issues posed by quantum computers.
% Supplemented by Schrödinger-style full-state simulations, researchers can attain a clearer view of the entire QAOA procedure. 
% Therefore, this paper emphasizes the stable QAOA experiments facilitated through our optimized simulator, using the typical Max-Cut problem as an illustrative case study.
% The overarching objective is to expedite the progress of QAOA, guiding it towards effectively tackling a wider spectrum of challenges.

==> contents/matrix_test.tex <==
\clearpage
$$
Rz_0z_1(\theta) = 
\begin{bmatrix}
e^{-i\frac{\theta}{2}} & 0 & 0 & 0 \\ 
0 & e^{i\frac{\theta}{2}}  & 0 & 0 \\
0 & 0 & e^{i\frac{\theta}{2}}  & 0 \\
0 & 0 & 0 & e^{-i\frac{\theta}{2}} \\
\end{bmatrix}
\otimes
\begin{bmatrix}
1 & 0 \\
0 & 1 \\
\end{bmatrix}
\rightarrow
\begin{bmatrix}
e^{i\frac{\theta}{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
0 & e^{i\frac{\theta}{2}}  & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & e^{-i\frac{\theta}{2}}  & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & e^{-i\frac{\theta}{2}}  & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & e^{-i\frac{\theta}{2}}  & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & e^{-i\frac{\theta}{2}}  & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & e^{i\frac{\theta}{2}}  & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & e^{i\frac{\theta}{2}} \\
\end{bmatrix}
$$

$$
Rz_1z_2(\theta) = 
\begin{bmatrix}
1 & 0 \\
0 & 1 \\
\end{bmatrix}
\otimes
\begin{bmatrix}
e^{-i\frac{\theta}{2}} & 0 & 0 & 0 \\ 
0 & e^{i\frac{\theta}{2}}  & 0 & 0 \\
0 & 0 & e^{i\frac{\theta}{2}}  & 0 \\
0 & 0 & 0 & e^{-i\frac{\theta}{2}} \\
\end{bmatrix}
\rightarrow
\begin{bmatrix}
e^{-i\frac{\theta}{2}} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
0 & e^{i\frac{\theta}{2}}  & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & e^{i\frac{\theta}{2}}  & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & e^{-i\frac{\theta}{2}}  & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & e^{-i\frac{\theta}{2}}  & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & e^{i\frac{\theta}{2}}  & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & e^{i\frac{\theta}{2}}  & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & e^{-i\frac{\theta}{2}} \\
\end{bmatrix}
$$
$$
tmpResult = Rz_0z_1(\theta)  Rz_1z_2(\theta) 
$$

$$
(\frac{2^N}{2^g}) * 2^{2g}Í \rightarrow (\frac{2^N}{2^g}) * 2^{g}
$$

$$
\textcolor{red}{C^N_2}
$$

\clearpage

==> figures/tmp_chap2.tex <==
\section{Background and Related Work}
\subsection{Parallel Computing}

Multiple Threading, such as OpenMP.

\textbf{Single Instruction Multiple Data(SIMD)}. 
Advanced Vector Extensions is an example.

\textbf{Single Instruction Multiple Thread(SIMT)}.
CUDA is an example.

\textbf{Quantum Computing(QC)}.

\begin{figure}[htb!]
\centerline{\includegraphics[scale=0.38]{figures/simd_simt2.pdf}}
\caption{test}
\label{fig:test}
\end{figure}

% ref: https://blog.csdn.net/qq_36653924/article/details/126543185

\subsection{Related Work of QAOA}

% The quantum approximation optimization algorithm, abbreviated as QAOA, is a hybrid algorithm to solve combinatorial optimization problem. 

% The algorithm can map a problem in QUBO form to the quantum circuits that output a solution to the problem. The circuits is parameterized by the variables $(\beta, \gamma)$ and has a depth of p.

% The hybird algorithm can be regarded as the process to get better solution through updating the parameter $(\beta, \gamma)$. The process is composed of a series of rounds. In each round, the circuits paramterized by $(\beta, \gamma)$ is executed and output a solution. Then, the classical computer will update the parameter $(\beta, \gamma)$ according to the solution and the parameter is fed to the next round.

% 下面的版本有 C 老師潤飾過

The Quantum Approximate Optimization Algorithm (QAOA), abbreviated as QAOA, is a hybrid algorithm designed to solve combinatorial optimization problems. 

It is special form of variational quantum eigensolvers, which approximate the ground energy state by updating the parameterize circuit.



The algorithm can map a problem in Quadratic Unconstrained Binary Optimization (QUBO) form to quantum circuits that output a solution to the problem. The circuits are parameterized by the variables $(\beta, \gamma)$ and have a depth of $p$. A higher $p$ leads to better approximation of the solution to the problem but incurs more computations.

The circuits starts with many H gates on each qubit to initialize the state to $\ket{+}^{\oplus N}$ 


The hybrid algorithm can be seen as a process of multiple iterations to improve the solution (i.e. find the lower energy state) by updating the parameters $(\beta, \gamma)$. In each iteration, the quantum circuits, with their parameters denoted as "$( \beta, \gamma)$," are run on either a quantum computer or a quantum simulator. Through this process, a solution is generated. The classical computer then updates the parameters $(\beta, \gamma)$ based on the obtained solution, which are subsequently used in the next iteration.

The circuit is composed of a series of H gates on each qubits as a initialization. Each round is composed of two layers, cost layer and mixer layer. The definition of two layers are shown below.

$$U_c (\gamma) = \prod e^{-i \gamma H_c}$$
$$U_m (\beta) = \prod e^{-i \beta H_m}$$

The $H_c$, cost Hamiltonian, is related to the problem solved. While the $H_m$, mixer Hamiltonian, is fixed to the following equation.

$$H_m = \sum_{i \in [0,N)} X_i$$
